Biased Agents, Extreme Beliefs: Motivated Reasoning Under Competing Models

People often face environments where multiple models compete to explain the same observations. This paper examines how people update beliefs in such settings and how preferences over payoff-relevant states shape model selection and belief updating. This paper first develops a framework where preference-driven bias distorts the perceived model, affecting Bayesian and best-fit updating differently. In a laboratory experiment, most participants are classified as Bayesian updaters, who average across models, while a substantial minority are classified as best-fit updaters, who select the model that best fits the observed signal. Within-participant comparisons between the symmetric payoff and asymmetric payoff conditions indicate that asymmetric payoffs shift reported beliefs toward the preferred state, particularly among participants classified as best-fit updaters. Relative to symmetric payoffs, asymmetric payoffs increase the reported belief of the preferred state by about 8 percentage points among best-fit updaters, while the estimated effect among Bayesian updaters is close to zero. These findings help us better understand model-based learning and have implications for domains such as political polarization and financial investment, where competing narratives and strong preferences often coexist.

==> NewTab/original_tab_individual_estimates_shared.tex <==
\begin{tabular}{lccccc}
\toprule
Type & 50\% Threshold & 90\% Threshold & Quiz & Cognitive Score & Overconfidence \\
\midrule
Bayesian & 132 & 118 & 9.55 & 2.82 & 72.0\% \\
Best-fit & 33 & 31 & 9.61 & 2.61 & 72.7\% \\
Non-mover & 28 & 18 & 9.21 & 2.61 & 85.7\% \\
\bottomrule
\end{tabular}


==> NewTab/tab_d02_existing_classification_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cc}}
\toprule
 & Participants & Share \\
\midrule
Bayesian & 132 & 0.684 \\
Best-fit & 33 & 0.171 \\
Non-mover & 28 & 0.145 \\
Unclassified participants & 0 & 0.000 \\
Classified at 70 percent threshold & 186 & 0.964 \\
Classified at 90 percent threshold & 167 & 0.865 \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r06_all_dp_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{2}{c}}
\toprule
DV: Reported Belief & (1) & (2) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP1}}\) & 0.027\sym{**} & 0.160\sym{***} \\
 & (0.011) & (0.050) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP2}}\) & 0.010 & 0.032 \\
 & (0.009) & (0.040) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP3}}\) & 0.009 & 0.049 \\
 & (0.010) & (0.045) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP4}}\) & 0.005 & 0.025 \\
 & (0.010) & (0.041) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP5}}\) & 0.012 & 0.041 \\
 & (0.011) & (0.033) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP6}}\) & 0.024\sym{**} & 0.127\sym{***} \\
 & (0.010) & (0.042) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP7}}\) & 0.023\sym{**} & 0.104\sym{***} \\
 & (0.010) & (0.038) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP8}}\) & 0.019\sym{**} & 0.078\sym{*} \\
 & (0.009) & (0.039) \\
\(\mathbbm{1}_{\text{Asym}}\) \(\times\mathbbm{1}_{\mathrm{DP9}}\) & 0.014 & 0.090\sym{**} \\
 & (0.009) & (0.038) \\
\midrule
Observations & 10422 & 1782 \\
Participants & 193 & 33 \\
Mean of DV & 0.506 & 0.476 \\
\(R^2\) & 0.511 & 0.377 \\
Sample & All participants & Best-fit \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r21_five1_preferred_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
DV: Reported Belief & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) & 0.016\sym{***} & 0.004 & 0.111\sym{***} & -0.004 & 0.012 & 0.021 \\
 & (0.005) & (0.003) & (0.024) & (0.009) & (0.015) & (0.114) \\
\midrule
Observations & 10422 & 6372 & 1242 & 1512 & 1026 & 270 \\
Participants & 193 & 118 & 23 & 28 & 19 & 5 \\
Mean of DV & 0.506 & 0.508 & 0.477 & 0.509 & 0.533 & 0.493 \\
\(R^2\) & 0.511 & 0.651 & 0.340 & 0.589 & 0.678 & 0.679 \\
Sample & All participants & Bayesian & Best-fit & Non-mover & Grether-Bayesian & Grether-Best-fit \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r21_five2_preferred_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{6}{c}}
\toprule
DV: Reported Belief & (1) & (2) & (3) & (4) & (5) & (6) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) & 0.016\sym{***} & 0.004 & 0.119\sym{***} & -0.003 & -0.010 & 0.006 \\
 & (0.005) & (0.003) & (0.023) & (0.006) & (0.022) & (0.041) \\
\midrule
Observations & 10422 & 6642 & 1188 & 1296 & 594 & 702 \\
Participants & 193 & 123 & 22 & 24 & 11 & 13 \\
Mean of DV & 0.506 & 0.512 & 0.472 & 0.509 & 0.505 & 0.511 \\
\(R^2\) & 0.511 & 0.659 & 0.367 & 0.738 & 0.358 & 0.559 \\
Sample & All participants & Bayesian & Best-fit & Non-mover & Grether-Bayesian A & Grether-Bayesian B \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r21_four_preferred_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{5}{c}}
\toprule
DV: Reported Belief & (1) & (2) & (3) & (4) & (5) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) & 0.016\sym{***} & 0.004 & 0.119\sym{***} & -0.004 & 0.006 \\
 & (0.005) & (0.003) & (0.023) & (0.009) & (0.041) \\
\midrule
Observations & 10422 & 6966 & 1188 & 1566 & 702 \\
Participants & 193 & 129 & 22 & 29 & 13 \\
Mean of DV & 0.506 & 0.511 & 0.472 & 0.510 & 0.511 \\
\(R^2\) & 0.511 & 0.638 & 0.367 & 0.575 & 0.559 \\
Sample & All participants & Bayesian & Best-fit & Non-mover & Grether-Bayesian \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r21_three_preferred.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
DV: Reported Belief & (1) & (2) & (3) & (4) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) & 0.016\sym{***} & 0.001 & 0.045\sym{***} & 0.002 \\
 & (0.005) & (0.003) & (0.014) & (0.002) \\
\midrule
Observations & 10422 & 6642 & 3402 & 378 \\
Participants & 193 & 123 & 63 & 7 \\
Mean of DV & 0.506 & 0.506 & 0.507 & 0.502 \\
\(R^2\) & 0.511 & 0.670 & 0.417 & 0.978 \\
Sample & All participants & Bayesian & Best-fit & Non-mover \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r21_two_preferred_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{3}{c}}
\toprule
DV: Reported Belief & (1) & (2) & (3) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) & 0.016\sym{***} & 0.003 & 0.083\sym{***} \\
 & (0.005) & (0.003) & (0.024) \\
\midrule
Observations & 10422 & 8694 & 1728 \\
Participants & 193 & 161 & 32 \\
Mean of DV & 0.506 & 0.512 & 0.476 \\
\(R^2\) & 0.511 & 0.599 & 0.370 \\
Sample & All participants & Bayesian & Best-fit \\
\bottomrule
\end{tabular}
}


==> NewTab/tab_r33_main_demographic_extremeness_full_shared.tex <==
{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{4}{c}}
\toprule
DV: Belief Extremeness & (1) & (2) & (3) & (4) \\
\midrule
\(\mathbbm{1}_{\text{Asym}}\) & -0.002 & 0.004 & -0.031\sym{**} & 0.004 \\
 & (0.003) & (0.003) & (0.013) & (0.007) \\
\midrule
Observations & 10422 & 7128 & 1782 & 1512 \\
Participants & 193 & 132 & 33 & 28 \\
Mean of DV & 0.176 & 0.164 & 0.276 & 0.116 \\
\(R^2\) & 0.251 & 0.407 & 0.098 & 0.450 \\
Sample & All participants & Bayesian & Best-fit & Non-mover \\
\bottomrule
\end{tabular}
}

